1st Place Solution for PSG competition with ECCV'22 SenseHuman Workshop

Panoptic Scene Graph (PSG) generation aims to generate scene graph representations based on panoptic segmentation instead of rigid bounding boxes. Existing PSG methods utilize one-stage paradigm which simultaneously generates scene graphs and predicts semantic segmentation masks or two-stage paradigm that first adopt an off-the-shelf panoptic segmentor, then pairwise relationship prediction between these predicted objects. One-stage approach despite having a simplified training paradigm, its segmentation results are usually under-satisfactory, while two-stage approach lacks global context and leads to low performance on relation prediction. To bridge this gap, in this paper, we propose GRNet, a Global Relation Network in two-stage paradigm, where the pre-extracted local object features and their corresponding masks are fed into a transformer with class embeddings. To handle relation ambiguity and predicate classification bias caused by long-tailed distribution, we formulate relation prediction in the second stage as a multi-class classification task with soft label. We conduct comprehensive experiments on OpenPSG dataset and achieve the state-of-art performance on the leadboard. We also show the effectiveness of our soft label strategy for long-tailed classes in ablation studies. Our code has been released in https://github.com/wangqixun/mfpsg.

==> latex/sections/20_Related_Work/manuscript.tex <==
\section{Related Works}

\subsection{Panoptic Scene Graph Generation}

\subsection{Global Contextual Modeling}

\subsection{Long-tailed Classification}

==> latex/sections/30_Method/fig_33.tex <==
\begin{figure}
\centering
\includegraphics[width=1\linewidth]{latex/figs/template.png}
\vspace{-3mm}
\caption{\textbf{Mult-label classification formlulation}.}
\label{fig_33}
\vspace{-3mm}
\end{figure}

==> latex/sections/30_Method/fig_34.tex <==
\begin{figure}[!tbp]
  \centering
  \includegraphics[width=1\linewidth]{latex/figs/Frequency_of_Predicates.png}
  \hfill
  \includegraphics[width=1\linewidth]{latex/figs/Frequency_of_Objects_(Thing).png}
  \caption{The long-tailed distribution of predicates and objects.}
\label{fig_34}
\end{figure}

==> latex/sections/40_Experiments/exp_pcl.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\centering
\begin{tabular}{|c|c|c|c|ccc|}
\hline
\multirow{2}{*}{Backbone}   & \multirow{2}{*}{Paradigm}   & \multirow{2}{*}{Segmentor}    & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Predicate Classification}                          \\ \cline{5-7} 
                            &                             &                               &                         & \multicolumn{1}{c|}{R/mR@20} & \multicolumn{1}{c|}{R/mR@50} & R/mR@100 \\ \hline
\multirow{6}{*}{ResNet-50}  & \multirow{16}{*}{Two-Stage} & \multirow{5}{*}{panoptic-fpn} & IMP                     & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & MOTIFS                  & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & VCTREE                  & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & GPSNet                  & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & GCNet                   & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{3-7} 
                            &                             & mask2former                   & GCNet                   & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{1-1} \cline{3-7} 
\multirow{6}{*}{ResNet-101} &                             & \multirow{5}{*}{panoptic-fpn} & IMP                     & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & MOTIFS                  & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & VCTREE                  & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & GPSNet                  & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{4-7} 
                            &                             &                               & GCNet                   & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{3-7} 
                            &                             & mask2former                   & GCNet                   & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{1-1} \cline{3-7} 
\multirow{2}{*}{Swin-Tiny}  &                             & panoptic-fpn                  & \multirow{4}{*}{GCNet}  & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{3-3} \cline{5-7} 
                            &                             & mask2former                   &                         & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{1-1} \cline{3-3} \cline{5-7} 
\multirow{2}{*}{Swin-Base}  &                             & panoptic-fpn                  &                         & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \cline{3-3} \cline{5-7} 
                            &                             & mask2former                   &                         & \multicolumn{1}{c|}{}        & \multicolumn{1}{c|}{}        &          \\ \hline
\end{tabular}
\caption{Comparison between all baselines and our GCNet. Recall (R) and mean recall (mR) are reported.}
\label{exp_pcl}
\end{table*}

==> latex/sections/40_Experiments/exp_sgg.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\centering
\begin{tabular}{|c|c|c|c|ccc|}
\hline
\multirow{2}{*}{Backbone}   & \multirow{2}{*}{Paradigm}  & \multirow{2}{*}{Segmentor}    & \multirow{2}{*}{Method} & \multicolumn{3}{c|}{Scene Graph Generation}                                       \\ \cline{5-7} 
                            &                            &                               &                         & \multicolumn{1}{c|}{R/mR@20}     & \multicolumn{1}{c|}{R/mR@50}     & R/mR@100    \\ \hline
\multirow{8}{*}{ResNet-50}  & \multirow{2}{*}{One-Stage} & \multirow{2}{*}{}             & PSGTR                   & \multicolumn{1}{c|}{28.4 / 16.6} & \multicolumn{1}{c|}{34.4 / 20.8} & 36.3 / 22.1 \\ \cline{4-7} 
                            &                            &                               & PSGFormer               & \multicolumn{1}{c|}{18.0 / 14.8} & \multicolumn{1}{c|}{19.6 / 17.0} & 20.1 / 17.6 \\ \cline{2-7} 
                            & \multirow{6}{*}{Two-Stage} & \multirow{5}{*}{panoptic-fpn} & IMP                     & \multicolumn{1}{c|}{16.5 / 6.52} & \multicolumn{1}{c|}{18.2 / 7.05} & 18.6 / 7.23 \\ \cline{4-7} 
                            &                            &                               & MOTIFS                  & \multicolumn{1}{c|}{20.0 / 9.10} & \multicolumn{1}{c|}{21.7 / 9.57} & 22.0 / 9.69 \\ \cline{4-7} 
                            &                            &                               & VCTREE                  & \multicolumn{1}{c|}{20.6 / 9.70} & \multicolumn{1}{c|}{22.1 / 10.2} & 22.5 / 10.2 \\ \cline{4-7} 
                            &                            &                               & GPSNet                  & \multicolumn{1}{c|}{17.8 / 7.03} & \multicolumn{1}{c|}{19.6 / 7.49} & 20.1 / 7.67 \\ \cline{4-7} 
                            &                            &                               & GCNet                   & \multicolumn{1}{c|}{31.0 / 25.9} & \multicolumn{1}{c|}{37.2 / 34.0} & 40.3 / 37.5 \\ \cline{3-7} 
                            &                            & mask2former                   & GCNet                   & \multicolumn{1}{c|}{38.1 / 32.6} & \multicolumn{1}{c|}{46.2 / 41.7} & 50.3 / 48.9 \\ \hline
\multirow{8}{*}{ResNet-101} & \multirow{2}{*}{One-Stage} & \multirow{2}{*}{}             & PSGTR                   & \multicolumn{1}{c|}{28.2 / 15.4} & \multicolumn{1}{c|}{32.1 / 20.3} & 35.3 / 21.5 \\ \cline{4-7} 
                            &                            &                               & PSGFormer               & \multicolumn{1}{c|}{18.6 / 16.7} & \multicolumn{1}{c|}{20.4 / 19.3} & 20.7 / 19.7 \\ \cline{2-7} 
                            & \multirow{6}{*}{Two-Stage} & \multirow{5}{*}{panoptic-fpn} & IMP                     & \multicolumn{1}{c|}{17.9 / 7.35} & \multicolumn{1}{c|}{19.5 / 7.88} & 20.1 / 8.02 \\ \cline{4-7} 
                            &                            &                               & MOTIFS                  & \multicolumn{1}{c|}{20.9 / 9.60} & \multicolumn{1}{c|}{22.5 / 10.1} & 23.1 / 10.3 \\ \cline{4-7} 
                            &                            &                               & VCTREE                  & \multicolumn{1}{c|}{21.7 / 9.68} & \multicolumn{1}{c|}{23.3 / 10.2} & 23.7 / 10.3 \\ \cline{4-7} 
                            &                            &                               & GPSNet                  & \multicolumn{1}{c|}{18.4 / 6.52} & \multicolumn{1}{c|}{20.0 / 6.97} & 20.6 / 7.17 \\ \cline{4-7} 
                            &                            &                               & GCNet                   & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-7} 
                            &                            & mask2former                   & GCNet                   & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \hline
\end{tabular}
\caption{Comparison between all baselines and our GCNet. Recall (R) and mean recall (mR) are reported.}
\label{exp_sgg}
\end{table*}

==> latex/sections/50_Ablation_Study/exp_ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[htb]
\centering
\begin{tabular}{|c|c|c|c|c|ccc|}
\hline
\multirow{2}{*}{Backbone}   & \multirow{2}{*}{Segmentor}   & \multirow{2}{*}{Global Context} & \multirow{2}{*}{Self-Distillation} & \multirow{2}{*}{Focal Loss} & \multicolumn{3}{c|}{Scene Graph Generation}                                       \\ \cline{6-8} 
                            &                              &                                 &                                    &                             & \multicolumn{1}{c|}{R/mR@20}     & \multicolumn{1}{c|}{R/mR@50}     & R/mR@100    \\ \hline
\multirow{5}{*}{ResNet-50}  & panoptic-fpn                 &                                 &                                    &                             & \multicolumn{1}{c|}{31.0 / 25.9} & \multicolumn{1}{c|}{37.2 /34.0}  & 40.3 / 37.5 \\ \cline{2-8} 
                            & \multirow{4}{*}{mask2former} & \times                          & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \checkmark                  & \multicolumn{1}{c|}{38.1 / 32.6} & \multicolumn{1}{c|}{46.2 / 41.7} & 50.3 / 48.9 \\ \hline
\multirow{5}{*}{ResNet-101} & panoptic-fpn                 &                                 &                                    &                             & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{2-8} 
                            & \multirow{4}{*}{mask2former} & \times                          & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \checkmark                  & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \hline
\multirow{5}{*}{Swin-Tiny}  & panoptic-fpn                 &                                 &                                    &                             & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{2-8} 
                            & \multirow{4}{*}{mask2former} & \times                          & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \checkmark                  & \multicolumn{1}{c|}{39.2 / 31.9} & \multicolumn{1}{c|}{47.7 / 43.2} & 51.9 / 49.5 \\ \hline
\multirow{5}{*}{Swin-Base}  & panoptic-fpn                 &                                 &                                    &                             & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{2-8} 
                            & \multirow{4}{*}{mask2former} & \times                          & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \times                             & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \times                      & \multicolumn{1}{c|}{}            & \multicolumn{1}{c|}{}            &             \\ \cline{3-8} 
                            &                              & \checkmark                      & \checkmark                         & \checkmark                  & \multicolumn{1}{c|}{40.8 / 34.2} & \multicolumn{1}{c|}{50.2 / 45.8} & 55.0 / 52.1 \\ \hline
\end{tabular}
\caption{The comparison of backbones and segmentors.}
\label{exp_ablation}
\end{table*}

==> latex/sections/50_Ablation_Study/manuscript.tex <==
\subsection{Ablation Study}
\label{Ablation Study}

We investigated the influence of different structure construction policies. They are reported on the Table \ref{exp_ablation}. 

\input{latex/sections/50_Ablation_Study/exp_ablation.tex}

\textbf{The Effectiveness of Global Context Modeling.}

\textbf{The Effectiveness of Self-Distillation.}

\textbf{The Effectiveness of Focal Loss.}
